Non-Causal Tracking by Deblatting

Tracking by Deblatting stands for solving an inverse problem of deblurring and image matting for tracking motion-blurred objects. We propose non-causal Tracking by Deblatting which estimates continuous, complete and accurate object trajectories. Energy minimization by dynamic programming is used to detect abrupt changes of motion, called bounces. High-order polynomials are fitted to segments, which are parts of the trajectory separated by bounces. The output is a continuous trajectory function which assigns location for every real-valued time stamp from zero to the number of frames. Additionally, we show that from the trajectory function precise physical calculations are possible, such as radius, gravity or sub-frame object velocity. Velocity estimation is compared to the high-speed camera measurements and radars. Results show high performance of the proposed method in terms of Trajectory-IoU, recall and velocity estimation.

==> figures/allspeed.tex <==
\begin{figure}
\centering
\begin{tabular}{cccc}

%% CSR-DCF
\resizebox {0.22\textwidth}{!} {\begin{tikzpicture}
\begin{axis}[legend style={fill=none},
  enlarge x limits=0.01,
    ybar=0pt,
    bar width=10,
    enlarge x limits={abs=0.5},
    ytick pos=left,
    xtick pos=left,
    area legend,
    ymax=1.0,ymin=0.0,xtick=data]
\addplot[fill=blue] coordinates {
(1, 0.3727)
(3, 0.3337)
(5, 0.2328)
(7, 0.1477)
(9, 0.0646)
};
\addplot[fill=cyan] coordinates {
(1, 0.7315)
(3, 0.7266)
(5, 0.5622)
(7, 0.3049)
(9, 0.1613)
};
\legend{TIoU, Recall}
\end{axis}
\end{tikzpicture}}

& 

%% FuCoLoT
\resizebox {0.22\textwidth}{!} {\begin{tikzpicture}
\begin{axis}[legend style={fill=none},
  enlarge x limits=0.01,
    ybar=0pt,
    bar width=10,
    enlarge x limits={abs=0.5},
    ytick pos=left,
    xtick pos=left,
    area legend,
    ymax=1.0,ymin=0.0,xtick=data]
\addplot[fill=blue] coordinates {
(1, 0.3366)
(3, 0.3054)
(5, 0.2315)
(7, 0.1571)
(9, 0.0644)
};
\addplot[fill=cyan] coordinates {
(1, 0.7407)
(3, 0.7302)
(5, 0.5484)
(7, 0.3293)
(9, 0.1613)
};
\legend{TIoU, Recall}
\end{axis}
\end{tikzpicture}}

&


%% FMOd
\resizebox {0.22\textwidth}{!} {\begin{tikzpicture}
\begin{axis}[legend style={fill=none},
  enlarge x limits=0.01,
    ybar=0pt,
    bar width=10,
    enlarge x limits={abs=0.5},
    ytick pos=left,
    xtick pos=left,
    area legend,
    ymax=1.0,ymin=0.0,xtick=data]
\addplot[fill=blue] coordinates {
(1, 0.1532)
(3, 0.3992)
(5, 0.3900)
(7, 0.2005)
(9, 0.0349)
};
\addplot[fill=cyan] coordinates {
(1, 0.2747)
(3, 0.5540)
(5, 0.5438)
(7, 0.3171)
(9, 0.0645)
};
\legend{TIoU, Recall}
\end{axis}
\end{tikzpicture}}

&

%% TbD-NC
\resizebox {0.22\textwidth}{!} {\begin{tikzpicture}
\begin{axis}[legend style={fill=none},
  enlarge x limits=0.01,
    ybar=0pt,
    bar width=10,
    enlarge x limits={abs=0.5},
    ytick pos=left,
    xtick pos=left,
    area legend,
    ymax=1.0,ymin=0.0,xtick=data]
\addplot[fill=blue] coordinates {
(1, 0.7479)
(3, 0.7087)
(5, 0.6092)
(7, 0.5939)
(9, 0.5490)
};
\addplot[fill=cyan] coordinates {
(1, 0.9321)
(3, 0.8993)
(5, 0.8341)
(7, 0.9268)
(9, 0.9677)
};
% \legend{TIoU, Recall}
\end{axis}
\end{tikzpicture}}

 \\

CSR-DCF~\cite{csrdcf} &  FuCoLoT~\cite{fucolot} & FMO algorithm~\cite{fmo} & TbD-NC \\

\end{tabular}
\caption[All-speed tracking]{All-speed tracking. Trajectory-IoU and recall on the extended TbD dataset (eTbD) for different algorithms (from left to right)~--~CSR-DCF~\cite{csrdcf}, FuCoLoT~\cite{fucolot}, FMO algorithm~\cite{fmo} and Tracking by Deblurring (TbD-NC). Horizontal axis denotes speed which is measured in radii per exposure. Vertical axis shows both success rates measured by TIoU and recall.}
\label{fig:allspeed}
\end{figure}



==> figures/deblurring.tex <==
\begin{figure}
	\noindent\begin{minipage}[t]{.24\linewidth}
		\centering
		\includegraphics[width=\textwidth]{imgs/deblurring/badminton_yellow_23_G}
	\end{minipage}\hfill%
	\begin{minipage}[t]{.24\linewidth}
		\centering
		\includegraphics[width=\textwidth]{imgs/deblurring/badminton_yellow_23_GT}
	\end{minipage}\hfill%
	\begin{minipage}[t]{.24\linewidth}
		\centering
		\includegraphics[width=\textwidth]{imgs/deblurring/badminton_yellow_23_H}
	\end{minipage}\hfill%
	\begin{minipage}[t]{.12\linewidth}
		\centering
		\includegraphics[width=\textwidth]{imgs/deblurring/badminton_yellow_23_F}
	\end{minipage}\hfill%
	\begin{minipage}[t]{.12\linewidth}
		\centering
		\includegraphics[width=\textwidth]{imgs/deblurring/badminton_yellow_23_M}
	\end{minipage}
	%
	\begin{minipage}[t]{.24\linewidth}
		\centering
		\includegraphics[width=\textwidth]{imgs/deblurring/volleyball_07_G}
	\end{minipage}\hfill%
	\begin{minipage}[t]{.24\linewidth}
		\centering
		\includegraphics[width=\textwidth]{imgs/deblurring/volleyball_07_GT}
	\end{minipage}\hfill%
	\begin{minipage}[t]{.24\linewidth}
		\centering
		\includegraphics[width=\textwidth]{imgs/deblurring/volleyball_07_H}
	\end{minipage}\hfill%
	\begin{minipage}[t]{.12\linewidth}
		\centering
		\includegraphics[width=\textwidth]{imgs/deblurring/volleyball_07_F}
	\end{minipage}\hfill%
	\begin{minipage}[t]{.12\linewidth}
		\centering
		\includegraphics[width=\textwidth]{imgs/deblurring/volleyball_07_M}
	\end{minipage}
	%
	\begin{minipage}[t]{.24\linewidth}
		\centering
		Input $I$
	\end{minipage}\hfill%
	\begin{minipage}[t]{.24\linewidth}
		\centering
		High FPS%
	\end{minipage}\hfill%
	\begin{minipage}[t]{.24\linewidth}
		\centering
		Blur $H$
	\end{minipage}\hfill%
	\begin{minipage}[t]{.12\linewidth}
		\centering
		$F$
	\end{minipage}\hfill%
	\begin{minipage}[t]{.12\linewidth}
		\centering
		$M$
	\end{minipage}%
	\caption[Deblatting examples]{Deblatting examples. From left to right: the input image, corresponding high-speed camera frame, estimated blur $H$, estimated appearance $F$ and shape $M$.}
	\label{fig:deblurring}
\end{figure}

==> figures/tbd_imgs.tex <==
\begin{figure}
\centering
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\raisebox{-.73\height}[0pt][0pt]{ 
\begin{tabular}{@{}r@{}}
\raisebox{44\height}[0pt][0pt]{1} \\
\raisebox{18\height}[0pt][0pt]{$\frac{1}{2}$}  \\
\raisebox{2\height}[0pt][0pt]{0} \\ 
\end{tabular}
\includegraphics[height=0.85\textwidth]{imgs/colormap_tiou.png}}
 & \input{imgs/tbd/badminton_white} & \input{imgs/tbd/badminton_yellow} &  \input{imgs/tbd/pingpong} \\
 & \input{imgs/tbd/tennis} &  \input{imgs/tbd/volleyball} & \input{imgs/tbd/throw_floor} \\
 & \input{imgs/tbd/throw_soft} & \input{imgs/tbd/throw_tennis} & \input{imgs/tbd/roll_golf} \\
 & \input{imgs/tbd/fall_cube} &   \input{imgs/tbd/hit_tennis} & \input{imgs/tbd/hit_tennis2}  \\
\end{tabular}

\caption{Trajectory recovery for selected sequences from the TbD dataset. Trajectory Intersection over Union (TIoU) with ground truth trajectories from a high-speed camera, color coded.
Arrows indicate the direction of the motion.
The trajectory over the whole sequence can be obtained by fitting a continuous piecewise quadratic curve~\eqref{eq:fitting_curve_def} on all frames jointly, as shown in the bottom right in blue.}
\label{fig:tbd_imgs}
\end{figure}


==> figures/tbd_lt_imgs.tex <==
\begin{figure}
\centering
\begin{tabular}{@{}c@{}c@{}c@{}}
\input{imgs/tbd_lt_nogt/badminton_white} & \input{imgs/tbd_lt_nogt/badminton_yellow} &  \input{imgs/tbd_lt_nogt/pingpong} \\
\input{imgs/tbd_lt_nogt/tennis} &  \input{imgs/tbd_lt_nogt/volleyball} &  \input{imgs/tbd_lt_nogt/throw_tennis} \\
% \input{imgs/tbd_lt/throw_soft} & \input{imgs/tbd_lt/throw_floor} & \input{imgs/tbd_lt/roll_golf} \\
% \input{imgs/tbd_lt/fall_cube} &   \input{imgs/tbd_lt/hit_tennis} & \input{imgs/tbd_lt/hit_tennis2}  \\
\end{tabular}

\caption[Trajectory recovery by TbD-NC on TbD dataset]{Trajectory recovery for selected sequences from the TbD dataset. Trajectory Intersection over Union (TIoU) with ground truth trajectories from a high-speed camera, color coded.
Arrows indicate the direction of the motion.}
\label{fig:tbd_lt_imgs}
\end{figure}

